Adversarial Sample-Based Approach for Tighter Privacy Auditing in Final Model-Only Scenarios

Auditing Differentially Private Stochastic Gradient Descent (DP-SGD) in the final model setting is challenging and often results in empirical lower bounds that are significantly looser than theoretical privacy guarantees. We introduce a novel auditing method that achieves tighter empirical lower bounds without additional assumptions by crafting worst-case adversarial samples through loss-based input-space auditing. Our approach surpasses traditional canary-based heuristics and is effective in final model-only scenarios. Specifically, with a theoretical privacy budget of $\varepsilon = 10.0$, our method achieves empirical lower bounds of $4.914$, compared to the baseline of $4.385$ for MNIST. Our work offers a practical framework for reliable and accurate privacy auditing in differentially private machine learning.

==> algorithms/auditing.tex <==
\begin{algorithm}[H]
    \small
    \caption{Auditing DP-SGD}\label{alg:audit_dpsgd}
    \begin{algorithmic}[1]
    \Require Training dataset $D$, DP-SGD mechanism $\mathcal{M}$, Canary sample $c$,  Loss function $\ell$, Number of observations $N$
    \State $D' = D \cup \{c\}$
    \State Observations $O \leftarrow \{\}$, $O' \leftarrow \{\}$
    \item[] \reduce
    \For{$i \in [N]$}
        \State $\theta_i \leftarrow \mathcal{M}(D)$
        \State $\theta'_i \leftarrow \mathcal{M}(D')$
        \State $O[i] \leftarrow \ell(\theta_i; c)$
        \State $O'[i] \leftarrow \ell(\theta'_i; c)$
    \EndFor \reduce
    \item[]
    \State \Return $\theta, O, O'$
    \color{black}
    \end{algorithmic}
\end{algorithm}
